Generalized Restart Mechanism for Successive-Cancellation Flip Decoding of Polar Codes

Polar codes are a class of linear error-correction codes that have received a lot of attention due to their ability to achieve channel capacity in an arbitrary binary discrete memoryless channel (B-DMC) with low-complexity successive-cancellation (SC) decoding. However, practical implementations often require better error-correction performance than what SC decoding provides, particularly at short to moderate code lengths. Successive-cancellation flip (SCF) decoding algorithm was proposed to improve error-correction performance with an aim to detect and correct the first wrongly estimated bit in a codeword before resuming SC decoding. At each additional SC decoding trial, i.e., decoding attempt beyond the initial unsuccessful trial, one bit estimated as the least reliable is flipped. Dynamic SCF (DSCF) is a variation of SCF, where multiple bits may be flipped simultaneously per trial. Despite the improved error-correction performance compared to the SC decoder, SCF-based decoders have variable execution time, which leads to high average execution time and latency. In this work, we propose the generalized restart mechanism (GRM) that allows to skip decoding computations that are identical between the initial trial and any additional trial. Under DSCF decoding with up to 3-bit flips per decoding trial, our proposed GRM is shown to reduce the average execution time by 25% to 60% without any negative effect on error-correction performance. The proposed mechanism is adaptable to state-of-the-art latency-reduction techniques. When applied to Fast-DSCF-3 decoding, the additional reduction brought by the GRM is 15% to 22%. For the DSCF-3 decoder, the proposed mechanism requires approximately 4% additional memory.

==> Distr_dscf3_N1024_5G_r025.tex <==
bfidx  distr
0	0.0140780181787369
1	0.0766350360297005
2	0.0456690787944841
3	0.000510433442219036
4	0.0697609284002935
5	0.0432265076306248
6	0.0273137704389017
7	0.0154124515316555
8	1.01477821514719e-06
9	0.0416728821832344
10	0.0254252681805128
11	0.0155809047153699
12	0.0646464461959516
13	0.00311739867693216
14	0.00166322149462624
15	0
16	0.00989510237590024
17	0.0433980051489847
18	0.00175962542506523
19	0.0264684601856841
20	0.000606837372658019
21	8.93004829329526e-05
22	0
23	0.0297624302720519
24	0.0160253775736044
25	4.97241325422122e-05
26	0.0101213979178781
27	1.52216732272078e-05
28	8.11822572117751e-06
29	0
30	0.00502518172140888
31	1.01477821514719e-06
32	0
33	0
34	0
35	0
36	0
37	0
38	0.0381607347806100
39	0.0212535149380427
40	0.0121306587838695
41	0.00729321103226284
42	0.00397590104694669
43	0
44	0.0247453667763642
45	0.0143580969661176
46	0.00796397943247514
47	0.0297096618048642
48	0.00145722151695136
49	0.0170604513530545
50	0.000413014733564906
51	6.19014711239785e-05
52	0
53	0.0283407259926307
54	0.00160842347100829
55	0.0207217711533056
56	0.0119632203783702
57	0.000122788164032810
58	0.0109017623653262
59	0.00637382196933949
60	5.07389107573594e-06
61	0.00330614742494954
62	1.01477821514719e-06
63	0
64	0
65	0.0110681859926104
66	0.00662853130134144
67	0.00381658086716858
68	0
69	0.00404389118736155
70	0.00256637410610724
71	0
72	0.00131007867575502
73	0
74	0
75	0
76	0.0164252001903724
77	0.000417073846425495
78	0.000213103425180910
79	0
80	0.000131921167969135
81	0
82	0
83	0
84	0.000112640381881338
85	0
86	0
87	0
88	0
89	0
90	0
91	0
92	0.00157392101169329
93	0.0130064123835415
94	0.00747282677634390
95	5.17536889725066e-05
96	0.00918577240351235
97	0.00555794028436115
98	0.00291139869925728
99	0
100	0.00309913266905951
101	0.00168453183714433
102	0
103	0.00108175357734690
104	0
105	0
106	0
107	0.00853124045474242
108	0.00507186151930565
109	0.00279469920451536
110	0.00180529044474685
111	0
112	0.00283326077669095
113	0.00162263036602035
114	0.000864591039305405
115	0
116	0.00660214706774761
117	0.000148157619411490
118	0.000103507377945013
119	0
120	7.81379225663335e-05
121	0
122	0
123	0
124	0.00108479791199234
125	0.00491761523060328
126	0.000120758607602515
127	9.23448175783942e-05
128	0
129	0.00233703422948398
130	1.72512296575022e-05
131	2.23251207332381e-05
132	0
133	1.01477821514719e-06
134	0
135	0
136	0
137	0.00155869933846608
138	1.42068950120606e-05
139	4.05911286058875e-06
140	0
141	1.01477821514719e-06
142	0
143	0
144	0
145	0
146	0
147	0
148	0
149	0
150	0
151	0
152	0
153	0.00158914268492050
154	0.000869664930381141
155	0.00407737886846140
156	0.000127862055108546
157	6.08866929088313e-05
158	0
159	0.00311435434228672
160	6.29162493391257e-05
161	0.00140851216262430
162	1.62364514423550e-05
163	0
164	0
165	0.000727595980260534
166	3.04433464544157e-06
167	1.01477821514719e-06
168	0
169	0
170	0
171	0
172	0
173	0.00190981260090701
174	0.000931566401505119
175	0
176	0.000426206850361819
177	0
178	0
179	0
180	0.000185704413371936
181	0
182	0
183	0
184	0
185	0
186	0
187	0
188	0.000116699494741927
189	0
190	0
191	0
192	0
193	0
194	0
195	0
196	0
197	0
198	0
199	0
200	0
201	0
202	0
203	0
204	0.000833132914635842
205	0.000379527052465049
206	0
207	0.000162364514423550
208	0
209	0
210	0
211	7.30640314905976e-05
212	0
213	0
214	0
215	0
216	0
217	0
218	0
219	4.46502414664763e-05
220	0
221	0
222	0
223	0
224	0
225	0
226	0
227	0
228	0
229	0
230	0
231	0
232	0
233	0
234	0
235	2.53694553786797e-05
236	0
237	0
238	0
239	0
240	0
241	0
242	0
243	0
244	0
245	0
246	0
247	0
248	0
249	0
250	0
251	0
252	0
253	0
254	0
255	0
256	0
257	0
258	0
259	0
260	0
261	0
262	0
263	0
264	0
265	0
266	0

==> Saved_cycles_N1024_First_Info.tex <==
bfidx  CyclesSavedP64  
0	367
1	367
2	367
3	367
4	367
5	367
6	367
7	367
8	367
9	367
10	367
11	367
12	367
13	367
14	367
15	367
16	367
17	367
18	367
19	367
20	367
21	367
22	367
23	367
24	367
25	367
26	367
27	367
28	367
29	367
30	367
31	367
32	367
33	367
34	367
35	367
36	367
37	367
38	367
39	367
40	367
41	367
42	367
43	367
44	367
45	367
46	367
47	367
48	367
49	367
50	367
51	367
52	367
53	367
54	367
55	367
56	367
57	367
58	367
59	367
60	367
61	367
62	367
63	367
64	367
65	367
66	367
67	367
68	367
69	367
70	367
71	367
72	367
73	367
74	367
75	367
76	367
77	367
78	367
79	367
80	367
81	367
82	367
83	367
84	367
85	367
86	367
87	367
88	367
89	367
90	367
91	367
92	367
93	367
94	367
95	367
96	367
97	367
98	367
99	367
100	367
101	367
102	367
103	367
104	367
105	367
106	367
107	367
108	367
109	367
110	367
111	367
112	367
113	367
114	367
115	367
116	367
117	367
118	367
119	367
120	367
121	367
122	367
123	367
124	367
125	367
126	367
127	367
128	367
129	367
130	367
131	367
132	367
133	367
134	367
135	367
136	367
137	367
138	367
139	367
140	367
141	367
142	367
143	367
144	367
145	367
146	367
147	367
148	367
149	367
150	367
151	367
152	367
153	367
154	367
155	367
156	367
157	367
158	367
159	367
160	367
161	367
162	367
163	367
164	367
165	367
166	367
167	367
168	367
169	367
170	367
171	367
172	367
173	367
174	367
175	367
176	367
177	367
178	367
179	367
180	367
181	367
182	367
183	367
184	367
185	367
186	367
187	367
188	367
189	367
190	367
191	367
192	367
193	367
194	367
195	367
196	367
197	367
198	367
199	367
200	367
201	367
202	367
203	367
204	367
205	367
206	367
207	367
208	367
209	367
210	367
211	367
212	367
213	367
214	367
215	367
216	367
217	367
218	367
219	367
220	367
221	367
222	367
223	367
224	367
225	367
226	367
227	367
228	367
229	367
230	367
231	367
232	367
233	367
234	367
235	367
236	367
237	367
238	367
239	367
240	367
241	367
242	367
243	367
244	367
245	367
246	367
247	367
248	367
249	367
250	367
251	367
252	367
253	367
254	367
255	367
256	367
257	367
258	367
259	367
260	367
261	367
262	367
263	367
264	367
265	367
266	367
267	367
268	367
269	367
270	367
271	367
272	367
273	367
274	367
275	367
276	367
277	367
278	367
279	367
280	367
281	367
282	367
283	367
284	367
285	367
286	367
287	367
288	367
289	367
290	367
291	367
292	367
293	367
294	367
295	367
296	367
297	367
298	367
299	367
300	367
301	367
302	367
303	367
304	367
305	367
306	367
307	367
308	367
309	367
310	367
311	367
312	367
313	367
314	367
315	367
316	367
317	367
318	367
319	367
320	367
321	367
322	367
323	367
324	367
325	367
326	367
327	367
328	367
329	367
330	367
331	367
332	367
333	367
334	367
335	367
336	367
337	367
338	367
339	367
340	367
341	367
342	367
343	367
344	367
345	367
346	367
347	367
348	367
349	367
350	367
351	367
352	367
353	367
354	367
355	367
356	367
357	367
358	367
359	367
360	367
361	367
362	367
363	367
364	367
365	367
366	367
367	367
368	367
369	367
370	367
371	367
372	367
373	367
374	367
375	367
376	367
377	367
378	367
379	367
380	367
381	367
382	367
383	367
384	367
385	367
386	367
387	367
388	367
389	367
390	367
391	367
392	367
393	367
394	367
395	367
396	367
397	367
398	367
399	367
400	367
401	367
402	367
403	367
404	367
405	367
406	367
407	367
408	367
409	367
410	367
411	367
412	367
413	367
414	367
415	367
416	367
417	367
418	367
419	367
420	367
421	367
422	367
423	367
424	367
425	367
426	367
427	367
428	367
429	367
430	367
431	367
432	367
433	367
434	367
435	367
436	367
437	367
438	367
439	367
440	367
441	367
442	367
443	367
444	367
445	367
446	367
447	367
448	367
449	367
450	367
451	367
452	367
453	367
454	367
455	367
456	367
457	367
458	367
459	367
460	367
461	367
462	367
463	367
464	367
465	367
466	367
467	367
468	367
469	367
470	367
471	367
472	367
473	367
474	367
475	367
476	367
477	367
478	367
479	367
480	367
481	367
482	367
483	367
484	367
485	367
486	367
487	367
488	367
489	367
490	367
491	367
492	367
493	367
494	367
495	367
496	367
497	367
498	367
499	367
500	367
501	367
502	367
503	367
504	367
505	367
506	367
507	367
508	367
509	367
510	367
511	367
512	367
513	367
514	367
515	367
516	367
517	367
518	367
519	367
520	367
521	367
522	367

==> Saved_cycles_N1024_P.tex <==
bfidx  CyclesSavedP64   CyclesSavedP16
0	346	347
1	537	538
2	538	539
3	630	630
4	632	632
5	633	633
6	661	662
7	672	673
8	677	678
9	679	680
10	680	681
11	695	696
12	700	701
13	702	703
14	703	704
15	710	711
16	711	712
17	713	714
18	714	715
19	718	719
20	719	720
21	721	722
22	722	723
23	910	923
24	915	928
25	917	930
26	918	931
27	971	983
28	994	1006
29	1005	1017
30	1010	1022
31	1012	1024
32	1013	1025
33	1041	1054
34	1052	1065
35	1056	1069
36	1057	1070
37	1059	1072
38	1060	1073
39	1072	1085
40	1074	1087
41	1075	1088
42	1079	1092
43	1080	1093
44	1082	1095
45	1083	1096
46	1090	1103
47	1091	1104
48	1093	1106
49	1094	1107
50	1098	1111
51	1099	1112
52	1101	1114
53	1102	1115
54	1163	1175
55	1186	1198
56	1196	1208
57	1197	1209
58	1201	1213
59	1202	1214
60	1204	1216
61	1205	1217
62	1232	1245
63	1233	1246
64	1241	1254
65	1243	1256
66	1244	1257
67	1248	1261
68	1249	1262
69	1251	1264
70	1252	1265
71	1264	1277
72	1266	1279
73	1267	1280
74	1271	1284
75	1272	1285
76	1274	1287
77	1275	1288
78	1282	1295
79	1283	1296
80	1285	1298
81	1286	1299
82	1290	1303
83	1291	1304
84	1293	1306
85	1294	1307
86	1320	1332
87	1325	1337
88	1327	1339
89	1328	1340
90	1336	1348
91	1338	1350
92	1339	1351
93	1343	1355
94	1344	1356
95	1346	1358
96	1347	1359
97	1359	1371
98	1361	1373
99	1362	1374
100	1366	1378
101	1367	1379
102	1369	1381
103	1370	1382
104	1377	1389
105	1378	1390
106	1380	1392
107	1381	1393
108	1385	1397
109	1386	1398
110	1388	1400
111	1389	1401
112	1405	1418
113	1406	1419
114	1408	1421
115	1409	1422
116	1413	1426
117	1414	1427
118	1416	1429
119	1417	1430
120	1424	1437
121	1425	1438
122	1427	1440
123	1428	1441
124	1432	1445
125	1433	1446
126	1435	1448
127	1436	1449
128	1447	1460
129	1448	1461
130	1450	1463
131	1451	1464
132	1455	1468
133	1456	1469
134	1458	1471
135	1459	1472
136	1466	1479
137	1467	1480
138	1469	1482
139	1470	1483
140	1474	1487
141	1475	1488
142	1477	1490
143	1478	1491
144	1593	1641
145	1640	1689
146	1663	1712
147	1674	1723
148	1679	1728
149	1681	1730
150	1682	1731
151	1735	1783
152	1758	1806
153	1768	1816
154	1769	1817
155	1773	1821
156	1774	1822
157	1776	1824
158	1777	1825
159	1797	1846
160	1802	1851
161	1804	1853
162	1805	1854
163	1813	1862
164	1815	1864
165	1816	1865
166	1820	1869
167	1821	1870
168	1823	1872
169	1824	1873
170	1836	1885
171	1838	1887
172	1839	1888
173	1843	1892
174	1844	1893
175	1846	1895
176	1847	1896
177	1854	1903
178	1855	1904
179	1857	1906
180	1858	1907
181	1862	1911
182	1863	1912
183	1865	1914
184	1866	1915
185	1924	1972
186	1926	1974
187	1927	1975
188	1942	1990
189	1947	1995
190	1949	1997
191	1950	1998
192	1958	2006
193	1960	2008
194	1961	2009
195	1965	2013
196	1966	2014
197	1968	2016
198	1969	2017
199	1989	2038
200	1994	2043
201	1996	2045
202	1997	2046
203	2005	2054
204	2007	2056
205	2008	2057
206	2012	2061
207	2013	2062
208	2015	2064
209	2016	2065
210	2027	2076
211	2028	2077
212	2030	2079
213	2031	2080
214	2035	2084
215	2036	2085
216	2038	2087
217	2039	2088
218	2046	2095
219	2047	2096
220	2049	2098
221	2050	2099
222	2054	2103
223	2055	2104
224	2057	2106
225	2058	2107
226	2084	2132
227	2089	2137
228	2091	2139
229	2092	2140
230	2099	2147
231	2100	2148
232	2102	2150
233	2103	2151
234	2107	2155
235	2108	2156
236	2110	2158
237	2111	2159
238	2122	2170
239	2123	2171
240	2125	2173
241	2126	2174
242	2130	2178
243	2131	2179
244	2133	2181
245	2134	2182
246	2141	2189
247	2142	2190
248	2144	2192
249	2145	2193
250	2149	2197
251	2150	2198
252	2152	2200
253	2153	2201
254	2169	2218
255	2170	2219
256	2172	2221
257	2173	2222
258	2177	2226
259	2178	2227
260	2180	2229
261	2181	2230
262	2188	2237
263	2189	2238
264	2191	2240
265	2192	2241
266	2196	2245
267	2197	2246
268	2199	2248
269	2200	2249
270	2211	2260
271	2212	2261
272	2214	2263
273	2215	2264
274	2219	2268
275	2220	2269
276	2222	2271
277	2223	2272
278	2230	2279
279	2231	2280
280	2233	2282
281	2234	2283
282	2238	2287
283	2239	2288
284	2241	2290
285	2242	2291
286	2288	2348
287	2299	2359
288	2304	2364
289	2306	2366
290	2307	2367
291	2322	2382
292	2327	2387
293	2329	2389
294	2330	2390
295	2337	2397
296	2338	2398
297	2340	2400
298	2341	2401
299	2345	2405
300	2346	2406
301	2348	2408
302	2349	2409
303	2368	2429
304	2369	2430
305	2373	2434
306	2374	2435
307	2376	2437
308	2377	2438
309	2384	2445
310	2385	2446
311	2387	2448
312	2388	2449
313	2392	2453
314	2393	2454
315	2395	2456
316	2396	2457
317	2407	2468
318	2408	2469
319	2410	2471
320	2411	2472
321	2415	2476
322	2416	2477
323	2418	2479
324	2419	2480
325	2426	2487
326	2427	2488
327	2429	2490
328	2430	2491
329	2434	2495
330	2435	2496
331	2437	2498
332	2438	2499
333	2461	2521
334	2463	2523
335	2464	2524
336	2468	2528
337	2469	2529
338	2471	2531
339	2472	2532
340	2479	2539
341	2480	2540
342	2482	2542
343	2483	2543
344	2487	2547
345	2488	2548
346	2490	2550
347	2491	2551
348	2502	2562
349	2503	2563
350	2505	2565
351	2506	2566
352	2510	2570
353	2511	2571
354	2513	2573
355	2514	2574
356	2521	2581
357	2522	2582
358	2524	2584
359	2525	2585
360	2529	2589
361	2530	2590
362	2532	2592
363	2533	2593
364	2549	2610
365	2550	2611
366	2552	2613
367	2553	2614
368	2557	2618
369	2558	2619
370	2560	2621
371	2561	2622
372	2568	2629
373	2569	2630
374	2571	2632
375	2572	2633
376	2576	2637
377	2577	2638
378	2579	2640
379	2580	2641
380	2591	2652
381	2592	2653
382	2594	2655
383	2595	2656
384	2599	2660
385	2600	2661
386	2602	2663
387	2603	2664
388	2610	2671
389	2611	2672
390	2613	2674
391	2614	2675
392	2618	2679
393	2619	2680
394	2621	2682
395	2622	2683
396	2653	2713
397	2655	2715
398	2656	2716
399	2660	2720
400	2661	2721
401	2663	2723
402	2664	2724
403	2671	2731
404	2672	2732
405	2674	2734
406	2675	2735
407	2679	2739
408	2680	2740
409	2682	2742
410	2683	2743
411	2694	2754
412	2695	2755
413	2697	2757
414	2698	2758
415	2702	2762
416	2703	2763
417	2705	2765
418	2706	2766
419	2713	2773
420	2714	2774
421	2716	2776
422	2717	2777
423	2721	2781
424	2722	2782
425	2724	2784
426	2725	2785
427	2741	2802
428	2742	2803
429	2744	2805
430	2745	2806
431	2749	2810
432	2750	2811
433	2752	2813
434	2753	2814
435	2760	2821
436	2761	2822
437	2763	2824
438	2764	2825
439	2768	2829
440	2769	2830
441	2771	2832
442	2772	2833
443	2783	2844
444	2784	2845
445	2786	2847
446	2787	2848
447	2791	2852
448	2792	2853
449	2794	2855
450	2795	2856
451	2802	2863
452	2803	2864
453	2805	2866
454	2806	2867
455	2810	2871
456	2811	2872
457	2813	2874
458	2814	2875
459	2836	2896
460	2837	2897
461	2839	2899
462	2840	2900
463	2844	2904
464	2845	2905
465	2847	2907
466	2848	2908
467	2855	2915
468	2856	2916
469	2858	2918
470	2859	2919
471	2863	2923
472	2864	2924
473	2866	2926
474	2867	2927
475	2878	2938
476	2879	2939
477	2881	2941
478	2882	2942
479	2886	2946
480	2887	2947
481	2889	2949
482	2890	2950
483	2897	2957
484	2898	2958
485	2900	2960
486	2901	2961
487	2905	2965
488	2906	2966
489	2908	2968
490	2909	2969
491	2925	2986
492	2926	2987
493	2928	2989
494	2929	2990
495	2933	2994
496	2934	2995
497	2936	2997
498	2937	2998
499	2944	3005
500	2945	3006
501	2947	3008
502	2948	3009
503	2952	3013
504	2953	3014
505	2955	3016
506	2956	3017
507	2967	3028
508	2968	3029
509	2970	3031
510	2971	3032
511	2975	3036
512	2976	3037
513	2978	3039
514	2979	3040
515	2986	3047
516	2987	3048
517	2989	3050
518	2990	3051
519	2994	3055
520	2995	3056
521	2997	3058
522	2998	3059

==> Saved_cycles_N1024_SRM.tex <==
bfidx  CyclesSavedP64  
0	0
1	0
2	0
3	0
4	0
5	0
6	0
7	0
8	0
9	0
10	0
11	0
12	0
13	0
14	0
15	0
16	0
17	0
18	0
19	0
20	0
21	0
22	0
23	0
24	0
25	0
26	0
27	0
28	0
29	0
30	0
31	0
32	0
33	0
34	0
35	0
36	0
37	0
38	0
39	0
40	0
41	0
42	0
43	0
44	0
45	0
46	0
47	0
48	0
49	0
50	0
51	0
52	0
53	0
54	0
55	0
56	0
57	0
58	0
59	0
60	0
61	0
62	0
63	0
64	0
65	0
66	0
67	0
68	0
69	0
70	0
71	0
72	0
73	0
74	0
75	0
76	0
77	0
78	0
79	0
80	0
81	0
82	0
83	0
84	0
85	0
86	0
87	0
88	0
89	0
90	0
91	0
92	0
93	0
94	0
95	0
96	0
97	0
98	0
99	0
100	0
101	0
102	0
103	0
104	0
105	0
106	0
107	0
108	0
109	0
110	0
111	0
112	0
113	0
114	0
115	0
116	0
117	0
118	0
119	0
120	0
121	0
122	0
123	0
124	0
125	0
126	0
127	0
128	0
129	0
130	0
131	0
132	0
133	0
134	0
135	0
136	0
137	0
138	0
139	0
140	0
141	0
142	0
143	0
144	1556
145	1556
146	1556
147	1556
148	1556
149	1556
150	1556
151	1556
152	1556
153	1556
154	1556
155	1556
156	1556
157	1556
158	1556
159	1556
160	1556
161	1556
162	1556
163	1556
164	1556
165	1556
166	1556
167	1556
168	1556
169	1556
170	1556
171	1556
172	1556
173	1556
174	1556
175	1556
176	1556
177	1556
178	1556
179	1556
180	1556
181	1556
182	1556
183	1556
184	1556
185	1556
186	1556
187	1556
188	1556
189	1556
190	1556
191	1556
192	1556
193	1556
194	1556
195	1556
196	1556
197	1556
198	1556
199	1556
200	1556
201	1556
202	1556
203	1556
204	1556
205	1556
206	1556
207	1556
208	1556
209	1556
210	1556
211	1556
212	1556
213	1556
214	1556
215	1556
216	1556
217	1556
218	1556
219	1556
220	1556
221	1556
222	1556
223	1556
224	1556
225	1556
226	1556
227	1556
228	1556
229	1556
230	1556
231	1556
232	1556
233	1556
234	1556
235	1556
236	1556
237	1556
238	1556
239	1556
240	1556
241	1556
242	1556
243	1556
244	1556
245	1556
246	1556
247	1556
248	1556
249	1556
250	1556
251	1556
252	1556
253	1556
254	1556
255	1556
256	1556
257	1556
258	1556
259	1556
260	1556
261	1556
262	1556
263	1556
264	1556
265	1556
266	1556
267	1556
268	1556
269	1556
270	1556
271	1556
272	1556
273	1556
274	1556
275	1556
276	1556
277	1556
278	1556
279	1556
280	1556
281	1556
282	1556
283	1556
284	1556
285	1556
286	1556
287	1556
288	1556
289	1556
290	1556
291	1556
292	1556
293	1556
294	1556
295	1556
296	1556
297	1556
298	1556
299	1556
300	1556
301	1556
302	1556
303	1556
304	1556
305	1556
306	1556
307	1556
308	1556
309	1556
310	1556
311	1556
312	1556
313	1556
314	1556
315	1556
316	1556
317	1556
318	1556
319	1556
320	1556
321	1556
322	1556
323	1556
324	1556
325	1556
326	1556
327	1556
328	1556
329	1556
330	1556
331	1556
332	1556
333	1556
334	1556
335	1556
336	1556
337	1556
338	1556
339	1556
340	1556
341	1556
342	1556
343	1556
344	1556
345	1556
346	1556
347	1556
348	1556
349	1556
350	1556
351	1556
352	1556
353	1556
354	1556
355	1556
356	1556
357	1556
358	1556
359	1556
360	1556
361	1556
362	1556
363	1556
364	1556
365	1556
366	1556
367	1556
368	1556
369	1556
370	1556
371	1556
372	1556
373	1556
374	1556
375	1556
376	1556
377	1556
378	1556
379	1556
380	1556
381	1556
382	1556
383	1556
384	1556
385	1556
386	1556
387	1556
388	1556
389	1556
390	1556
391	1556
392	1556
393	1556
394	1556
395	1556
396	1556
397	1556
398	1556
399	1556
400	1556
401	1556
402	1556
403	1556
404	1556
405	1556
406	1556
407	1556
408	1556
409	1556
410	1556
411	1556
412	1556
413	1556
414	1556
415	1556
416	1556
417	1556
418	1556
419	1556
420	1556
421	1556
422	1556
423	1556
424	1556
425	1556
426	1556
427	1556
428	1556
429	1556
430	1556
431	1556
432	1556
433	1556
434	1556
435	1556
436	1556
437	1556
438	1556
439	1556
440	1556
441	1556
442	1556
443	1556
444	1556
445	1556
446	1556
447	1556
448	1556
449	1556
450	1556
451	1556
452	1556
453	1556
454	1556
455	1556
456	1556
457	1556
458	1556
459	1556
460	1556
461	1556
462	1556
463	1556
464	1556
465	1556
466	1556
467	1556
468	1556
469	1556
470	1556
471	1556
472	1556
473	1556
474	1556
475	1556
476	1556
477	1556
478	1556
479	1556
480	1556
481	1556
482	1556
483	1556
484	1556
485	1556
486	1556
487	1556
488	1556
489	1556
490	1556
491	1556
492	1556
493	1556
494	1556
495	1556
496	1556
497	1556
498	1556
499	1556
500	1556
501	1556
502	1556
503	1556
504	1556
505	1556
506	1556
507	1556
508	1556
509	1556
510	1556
511	1556
512	1556
513	1556
514	1556
515	1556
516	1556
517	1556
518	1556
519	1556
520	1556
521	1556
522	1556

==> dscf1_exec_av_N1024_5G_R05.tex <==
EbN0  fer execav execavgrm
0.2500 0.99206 24575.254464 19982.223214
0.3750 0.97371 24333.335930 19694.007303
0.5000 0.95877 24038.791467 19387.185523
0.6250 0.92293 23411.965390 18798.833872
0.7500 0.86244 22419.975420 17898.332040
0.8750 0.80257 21303.759631 16874.012039
1.0000 0.68823 19330.892292 15224.327942
1.1250 0.56705 16744.440885 13147.160193
1.2500 0.45903 14654.991049 11475.482672
1.3750 0.34632 12304.774026 9643.265455
1.5000 0.23652 9851.492313 7799.334082
1.6250 0.15288 7856.706467 6330.171763
1.7500 0.09205 6271.452918 5211.310199
1.8750 0.05237 5117.500772 4397.798136
2.0000 0.02856 4359.167664 3890.649051
2.1250 0.01423 3843.712385 3552.549427
2.2500 0.00698 3529.234170 3352.781345
2.3750 0.00359 3346.935495 3241.937240
2.5000 0.00160 3239.214255 3177.176060
2.6250 0.00065 3177.513165 3140.686490
2.7500 0.00033 3141.874665 3120.879315
2.8750 0.00019 3124.365315 3111.741455
3.0000 0.00009 3113.704755 3106.197540

==> dscf2_exec_av_N1024_5G_R05.tex <==
EbN0  fer execav execavgrm
0.2500 0.98668 153185.695116 120607.844598
0.3750 0.95012 149912.100713 117446.566746
0.5000 0.93066 147764.184737 115204.136342
0.6250 0.86919 139631.431551 108156.505432
0.7500 0.78771 129723.480898 99837.910595
0.8750 0.69735 117499.427824 89486.699093
1.0000 0.54825 97112.194079 73438.037829
1.1250 0.42680 79617.053137 59571.001280
1.2500 0.30139 61025.455696 45459.366486
1.3750 0.19726 43332.205346 32013.617714
1.5000 0.11896 29567.589782 21891.767739
1.6250 0.06332 18621.472534 13919.073801
1.7500 0.03261 12046.714412 9201.769934
1.8750 0.01471 7953.925993 6334.425408
2.0000 0.00639 5611.328310 4729.567265
2.1250 0.00294 4416.725790 3930.155915
2.2500 0.00113 3763.843965 3501.440815
2.3750 0.00039 3433.630020 3295.612540
2.5000 0.00016 3276.541710 3198.133045

==> dscf3_Fast_exec_av_N1024_5G_R025.tex <==
EbN0  fer  execav  execavgrm
0.2500 0.35311 86398.977754 71750.319386
0.3750 0.27097 68398.687170 55981.031568
0.5000 0.18486 49945.961549 40531.088271
0.6250 0.11923 33729.371110 27083.552164
0.7500 0.07483 22912.694803 18159.583867
0.8750 0.04429 14595.419243 11459.465102
1.0000 0.02439 8929.584403 6947.224527
1.1250 0.01295 5470.117313 4259.311055
1.2500 0.00642 3367.126230 2649.599635
1.3750 0.00298 2070.868995 1672.405170
1.5000 0.00132 1446.117075 1220.514790
1.6250 0.00056 1090.748295 968.293270
1.7500 0.00027 935.482860 866.398515
1.8750 0.00009 841.753770 802.751935
2.0000 0.00007 800.631975 776.143460

==> dscf3_PLRT_exec_av_N1024_5G_R025.tex <==
EbN0 SNR  fer  execavplrt  execavplrtgrm
0.2500    -2.7603 0.35311 273888.257415 193364.456391
0.3750    -2.6353 0.27097 216826.607506 150196.934562
0.5000    -2.5103 0.18486 158330.720214 108608.560033
0.6250    -2.3853 0.11923 106923.471980 72479.028437
0.7500    -2.2603 0.07483 72634.170165 48536.532757
0.8750    -2.1353 0.04429 46268.069907 30666.567737
1.0000    -2.0103 0.02439 28307.144080 18670.685614
1.1250    -1.8853 0.01295 17340.493346 11562.438970
1.2500    -1.7603 0.00642 10673.926470 7322.443970
1.3750    -1.6353 0.00298 6564.738555 4760.469245
1.5000    -1.5103 0.00132 4584.249675 3582.825715
1.6250    -1.3853 0.00056 3457.716255 2928.674625
1.7500    -1.2603 0.00027 2965.518540 2669.003590
1.8750    -1.1353 0.00009 2668.393530 2505.625950
2.0000    -1.0103 0.00007 2538.035775 2437.821880

==> dscf3_exec_av_N1024_5G_R0125.tex <==
EbN0  SNR fer  execav execavsrm  execavgrm
0.2500 -5.7706 0.18442 207719.869156 148265.747626 80162.012909
0.3750 -5.6456 0.13986 162522.178951 114244.177832 61910.050769
0.5000 -5.5206 0.10092 123404.378715 86227.465964  46918.638290
0.6250 -5.3956 0.06698 86472.665952 59922.067520   32883.070701
0.7500 -5.2706 0.04499 63038.373642 43370.760443   24162.210810
0.8750 -5.1456 0.02919 44253.656667 30503.391081   17303.694460
1.0000 -5.0206 0.01784 29168.647227 20130.314138   11829.727690
1.1250 -4.8956 0.01085 20340.211881 14227.221519   8766.357355
1.2500 -4.7706 0.00611 13568.258730 9737.192230    6446.483195
1.3750 -4.6456 0.00358 9735.446520 7259.702700     5169.726680
1.5000 -4.5206 0.00186 6963.375525 5489.221125     4272.227070
1.6250 -4.3956 0.00118 5518.389300 4576.013460     3818.091185
1.7500 -4.2706 0.00047 4518.078585 3957.980825     3507.455110
1.8750 -4.1456 0.00032 3981.781140 3624.282360     3345.673445
2.0000 -4.0206 0.00019 3654.278820 3427.141720     3250.600200

==> dscf3_exec_av_N1024_5G_R025.tex <==
EbN0  SNR fer  execav execavsrm  execavgrm
0.2500 -2.7603 0.35311 361336.615466 324139.589336  194114.456391
0.3750 -2.6353 0.27097 286056.047961 251270.246037  150946.934562
0.5000 -2.5103 0.18486 208883.312875 181784.837231  109358.560033
0.6250 -2.3853 0.11923 141062.511566 121090.350841  73229.028437
0.7500 -2.2603 0.07483 95825.156808 81012.854192   49286.532757
0.8750 -2.1353 0.04429 61040.761448 50975.171103   31416.567737
1.0000 -2.0103 0.02439 37345.184974 30806.179256  19420.685614
1.1250 -1.8853 0.01295 22877.049331 18785.075780  12312.438970
1.2500 -1.7603 0.00642 14081.948970 11609.161550  8072.443970
1.3750 -1.6353 0.00298 8660.759805 7279.965405    5510.469245
1.5000 -1.5103 0.00132 6047.930925 5255.047785   4332.825715
1.6250 -1.3853 0.00056 4561.712505 4130.443765   3678.674625
1.7500 -1.2603 0.00027 3912.363540 3671.074620   3419.003590
1.8750 -1.1353 0.00009 3520.371030 3386.204930   3255.625950
2.0000 -1.0103 0.00007 3348.392025 3265.628385   3187.821880

==> dscf3_exec_av_N1024_5G_R05.tex <==
EbN0  fer execav execavsrm execavgrm
0.2500 0.97466 836418.891813 835979.845029  655844.375731
0.3750 0.92807 818074.163805 817417.827842  638124.412065
0.5000 0.89166 788859.223362 787593.889434  612687.211770
0.6250 0.79745 727010.819378 725118.554625  561814.397927
0.7500 0.69954 647340.885624 644887.967821 496767.641833
0.8750 0.58600 557671.996191 553793.165837  423496.614415
1.0000 0.43422 424016.671733 420275.312636 319808.905341
1.1250 0.31551 330535.067203 326743.621234  247514.470894
1.2500 0.19372 218544.938009 215202.190624   162339.279155
1.3750 0.11540 138355.660550 135522.072414  101893.420345
1.5000 0.06179 80857.093698 78761.372722  59245.796880
1.6250 0.02978 44637.854629 43086.673257  32625.526576
1.7500 0.01267 23340.714039 22396.810709  17274.436270
1.8750 0.00518 12377.220060 11806.144720  9444.474600
2.0000 0.00210 7458.301320 7127.690220  6006.800985
2.1250 0.00086 5016.785160 4819.624400  4328.752775
2.2500 0.00024 3984.120885 3875.597665  3649.163325
2.3750 0.00010 3483.802830 3422.706490  3325.474480

==> scf_exec_av_N1024_5G_R05.tex <==
EbN0  fer execav execavgrm
0.2500 0.99108 39924.579782 20535.662042
0.3750 0.97466 39409.554094 20104.026316
0.5000 0.95740 38994.884634 19762.191000
0.6250 0.91743 37948.534404 19119.252752
0.7500 0.85837 36141.256223 18101.037768
0.8750 0.80032 34279.974790 17126.412965
1.0000 0.70746 31520.568093 15681.548638
1.1250 0.58497 27164.062884 13676.442527
1.2500 0.48450 23798.037791 12096.418362
1.3750 0.38183 19902.111684 10327.873998
1.5000 0.28007 15924.633105 8568.006022
1.6250 0.19316 12543.557176 7098.400715
1.7500 0.13170 9955.124259 6007.859542
1.8750 0.08527 7773.659703 5061.984055
2.0000 0.05198 6162.644984 4374.529080
2.1250 0.03052 5026.352438 3898.629999
2.2500 0.01690 4264.194885 3583.370110
2.3750 0.00894 3773.822745 3377.770850
2.5000 0.00460 3474.722760 3254.933100
2.6250 0.00243 3316.828710 3188.651005
2.7500 0.00105 3208.875045 3143.769875
2.8750 0.00044 3155.076405 3121.507425
3.0000 0.00023 3131.353560 3112.361580

==> scl_l8_N1024_R05_5G.tex <==
EbN0  fer  
0.25    0.921234   
0.375   0.834028  
0.5     0.759013 
0.625   0.651254  
0.75    0.543183   
0.875   0.406091   
1       0.298864  
1.125   0.195274  
1.25     0.123609  
1.375   0.0720279 
1.5     0.0408305  
1.625   0.0208444  
1.75    0.00972   
1.875  0.004385  
2       0.001975   
2.125   0.00073   
2.25   0.00034   
2.375    0.00012   
